Equivariant Filter Design for Inertial Navigation Systems with Input Measurement Biases

Inertial Navigation Systems (INS) are a key technology for autonomous vehicles applications. Recent advances in estimation and filter design for the INS problem have exploited geometry and symmetry to overcome limitations of the classical Extended Kalman Filter (EKF) approach that formed the mainstay of INS systems since the mid-twentieth century. The industry standard INS filter, the Multiplicative Extended Kalman Filter (MEKF), uses a geometric construction for attitude estimation coupled with classical Euclidean construction for position, velocity and bias estimation. The recent Invariant Extended Kalman Filter (IEKF) provides a geometric framework for the full navigation states, integrating attitude, position and velocity, but still uses the classical Euclidean construction to model the bias states. In this paper, we use the recently proposed Equivariant Filter (EqF) framework to derive a novel observer for biased inertial-based navigation in a fully geometric framework. The introduction of virtual velocity inputs with associated virtual bias leads to a full equivariant symmetry on the augmented system. The resulting filter performance is evaluated with both simulated and real-world data, and demonstrates increased robustness to a wide range of erroneous initial conditions, and improved accuracy when compared with the industry standard Multiplicative EKF (MEKF) approach.

==> preamble/preamble_compatible.tex <==

% Colour.  Used mostly for todos/notes/audits.
\usepackage{xcolor}  % Needed for colours - load before mdframed

%% RM Commenting process
%===================================================
%% comment environments {audit}
% audit.  Its an environment used for large chunks of text
\newenvironment{audit}{\color{orange}}{\color{black}}
% todo - use for a reminder of things to do.
\newcommand{\todo}[1]{{\color{red} #1}}
%% aside - a short comment to the authors, but not requiring work.
\newcommand{\aside}[1]{{\color{blue} #1}}
%% \margin{...} % a very short comment put in the margin.
\newcommand{\margin}[1]{\marginpar{\tiny #1}}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Uncomment to switch off notes
%\renewcommand{\margin}[1]{} %% Get rid of all margin comments
%\renewcommand{\todo}[1]{}%%  Get rid of todo comments
%\renewenvironment{audit}{}{} %% leave the audit text but without the colour.
%\renewcommand{\aside}[1]{} %% Get rid of all comments
%===================================================

% math symbols 
\usepackage{amssymb}
% We did use MnSymbol but this had problems with type 3 fonts.

\usepackage{amsmath}
\usepackage{mathdots}

%  this is used for \mathclap and symbol generation needed for \obb symbol.
\usepackage{mathtools} 

% for \mathbb
%\usepackage{bbm}
%\let\mathbb\mathbbm

% left indices
\usepackage{tensor}

% for \mathcal lower case
\usepackage{urwchancal}
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% allow the use of scalable vector graphics
\usepackage{graphicx}
\usepackage{ifpdf}
\ifpdf
\usepackage{epstopdf}
\epstopdfsetup{update,prepend}
\PrependGraphicsExtensions{.svg}
\DeclareGraphicsRule{.svg}{pdf}{.pdf}{% <- do not remove!
  `inkscape -z -D #1 --export-pdf=\noexpand\OutputFile
}
\fi
%% To switch off figures -
%\usepackage[demo]{graphicx} % use this to switch off figures


% theorem environments
%\usepackage{amsthm}
% -- or
%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

% list environments
\newenvironment{List}
{\begin{list}
 {[\arabic{enumi}]}
 {\usecounter{enumi}
  \settowidth{\labelwidth}{[99]}}
  \setlength{\labelsep}{1em}}
{\end{list}}


==> sections/acknowledgement.tex <==
\section*{Acknowledgement}

==> sections/simulations.tex <==
\section{Experiments}\label{sec:sim}

To validate the proposed \acl{eqf} design for a \acl{bins}, we performed different simulations, as well as, real-world experiments, of a \ac{uav} carrying an \ac{imu} and receiving extended pose measurements. The simulated \ac{uav} is navigating a spline interpolated trajectory passing through randomly chosen waypoints, that provides ground-truth values for the \ac{uav} position, orientation, velocity and acceleration. These values were used to generate simulated extended pose measurements as well as simulated \ac{imu} measurements affected by slowly time-varying biases. In order to replicate a real-world scenario, zero mean white Gaussian noise was added to both the simulated extended pose and the \ac{imu} measurements.

\begin{table}[!ht]
\renewcommand{\arraystretch}{1.15}
\setlength\tabcolsep{4.5pt}
\centering
\scriptsize
\caption{}
\vspace{-5pt}
\begin{tabular}{c c c c c c}
\specialrule{.1em}{.1em}{.1em} 
\textsc{Rmse} & Att [\si[per-mode = symbol]{\degree}]& Pos [\si[per-mode = symbol]{\meter}] & Vel [\si[per-mode = symbol]{\meter\per\second}] & Gyro bias [\si[per-mode = symbol]{\radian\per\second}] & Acc bias [\si[per-mode = symbol]{\meter\per\square\second}] \\ \hline
\ac{eqf} & $\mathbf{0.1549}$ & $\mathbf{0.0445}$ & $\mathbf{0.0146}$ & $\mathbf{0.0009}$ & $\mathbf{0.043}$ \\
\ac{ekf} & $0.3507$ & $0.0486$ & $0.0438$ & $0.0043$ & $0.0867$\\
\specialrule{.1em}{.1em}{.1em} 
\end{tabular}
\label{tab:rmse}
%\vspace{-10pt}
\end{table}

In all the simulations and real-world experiments, the state origin ${\xi_{0}}$ was chosen to be the identity of the state space, leading to an identity output origin $y_{0}$. The state and the output gain matrix for the \acl{eqf} were selected to reflect input and output measurements noise respectively.

Each simulation covers a time span of \SI{60}{\second} with \ac{imu} and extended pose measurements provided at \SI{500}{\hertz}. Biases are simulated to have slowly time-varying dynamics.%, and a ground-truth value with an average of ${\Vector{I}{b_{\bm{\omega}}}{} = \left[0.04\;\, 0.08\;\, 0.019\right]^T}$, ${\Vector{I}{b_{\bm{\nu}}}{} = \mathbf{0}^T}$ and ${\Vector{I}{b_{\bm{a}}}{} = \left[0.094\;\, 0.11\;\, 0.14\right]^T}$.
The standard deviation of the measurement noise values are ${\sigma_{\Vector{}{w}{}} = 1.75\cdot10^{-6}}$\si[per-mode = symbol]{\radian\per\second}, and ${\sigma_{\Vector{}{a}{}} = 1\cdot10^{-3}}$\si[per-mode = symbol]{\meter\per\square\second} for simulated \ac{imu} measurements reflecting real MEMS-type \ac{imu} values and ${\sigma_{\Vector{}{\theta}{}} = 1.75\cdot10^{-2}}$\si[per-mode = symbol]{\radian}, ${\sigma_{\Vector{}{p}{}} = 0.1}$\si[per-mode = symbol]{\meter} and ${\sigma_{\Vector{}{v}{}} = 0.05}$\si[per-mode = symbol]{\meter\per\second} for extended pose measurements.

Every time a set of measurements is received, the input of the system is set to $\bm{u} = \left(\Vector{I}{w}{}^{\wedge}, \Vector{}{g}{}^{\wedge}, \mathbf{0}^{\wedge} \right)$, and the \acl{eqf} and Riccati dynamics in \equref{observerode1}-\eqref{eq:riccatiode} are integrated using a Runge-Kutta method with MATLAB's ode45 solver.

In the first simulation setup, we ran the proposed \ac{eqf} and a Multiplicative \ac{ekf} on 10 different trajectories. Both filters were initialized with  identity orientation, zero position, velocity, and biases. The initial value for the Riccati matrix was chosen to reflect the initial error. In \figref{traj}, the \ac{uav} simulated trajectory and the filters estimate for one of the 10 runs are shown. Furthermore, \tabref{rmse} reports a comparison of the \acs{rmse} of navigation states and biases for the two filters computed for the second half of the trajectory (when both filters converged), averaged over the 10 runs, showing the improved accuracy of the proposed \ac{eqf}.

To show the robustness of the proposed methodology to different initial conditions, in the second simulation setup, we ran a batch of 10 different runs of the same trajectory, where the initialization of the \ac{eqf} varies from a perfect initialization to an extremely wrong initialization with an error of up to three orders of magnitude ($10^3$). Along these runs the initial value for the Riccati matrix was increased with the initialization error. \figref{logerrors} shows the evolution of the logarithm of the Equivariant error in \equref{local_coord_xi} for the 9 experiments with incorrect filter initialization. Note that even when the filter is initialized with extremely high error, in the order of $10^3$ for both biases and navigation states, it still converges and provides good estimates with an error smaller than $10^{-2}$ in any of the states. Moreover, the exponential convergence of the equivariant error is shown in \figref{lyap} by the time evolution of the Lyapunov function (Filter energy) $\calL_t$ for the different runs with different filter initialization. 

Furthermore, the proposed \ac{eqf} was evaluated, and compared with a Multiplicative \ac{ekf}, on real-world in-flight data. Raw \ac{imu} readings were recorded at \SI{200}{\hertz} on a AscTec Hummingbird quadcopter flying a Lissajous surve, and raw pose measurements gathered at \SI{30}{\hertz} from a OptiTrack motion capture system. Velocity measurements were derived by numerical differentiation of the filtered position measurements. The extended pose measurements at \SI{30}{\hertz} were then interpolated to obtain extended pose measurements at \SI{200}{\hertz} coinciding with the \ac{imu} readings, and finally added with zero mean white Gaussian noise. Standard deviation of the \ac{imu} measurement noise values was set to proper values determined using Allan Variance. Extended pose measurements standard deviation was set to ${\sigma_{\Vector{}{\theta}{}} = 0.0175}$ $\text{rad}$, ${\sigma_{\Vector{}{p}{}} = 0.1}$ $\text{m}$ and ${\sigma_{\Vector{}{v}{}} = 0.05}$ $\text{m/s}$. 
%
%Results, in \figref{real_world_trajectories}, and \tabref{rmse_L} show slightly improved performance
%\footnote{Note that, the results achieved by the \ac{eqf} are relevant given the fact that the problem of estimating the state of the biased inertial navigation system with full navigation state measurement is very well posed, and \ac{ekf}s are known to work well in practice.}
%\footnote{Note that, even though the proposed \ac{eqf} only slightly outperform the \ac{ekf}, the results achieved by the \ac{eqf} are still relevant given the fact that the problem of estimating the state of the biased inertial navigation system with full navigation state measurement is very well posed, and \ac{ekf}s are known to work well in practice.} 
%of the \ac{eqf} compared to the \ac{ekf} for the navigation states, on the real-world in-flight data. Instead, results of biases estimation cannot be compared due to a lack of ground-truth data.
%
Results, in \figref{real_world_trajectories}, and \tabref{rmse_L} the performance (RMSE)
of the \ac{eqf} compared to the \ac{ekf} for the navigation states on the real-world in-flight data. Note that there is no ground-truth for the bias states, hence we omitted the corresponding values. The slight performance improvement is accompanied with the benefit of a tightly-coupled geometrical description of biases and navigation states for improved bias estimation (see \tabref{rmse}).
% 



\begin{figure}[!t]
\centering
\includegraphics[width=.99\linewidth]{images/trajectory}
\vspace{-20pt}
\caption{Simulated \ac{uav} trajectory plot, showing in light green the ground-truth and in red and blue the \ac{eqf} and \ac{ekf} estimate respectively. In this experiment the filter was wrongly initialized with an identity extended pose and zero biases, whereas the ground-truth trajectory started at ${\Vector{G}{p}{I} = \left[4.58\;4.6\;3.91\right]^T}$, ${\Vector{G}{v}{I} = \left[-0.97\;2.43\;9.29\right]^T}$, with initial orientation of ${\Vector{G}{\theta}{I} = \left[1.92\;-32.06\;-8.95\right]^T}$ intended as yaw-pitch-roll angles in degree, with biases ${\Vector{I}{b_{\bm{\omega}}}{} = \left[0.04\;\, 0.08\;\, 0.019\right]^T}$, ${\Vector{I}{b_{\bm{\nu}}}{} = \mathbf{0}^T}$ and ${\Vector{I}{b_{\bm{a}}}{} = \left[0.094\;\, 0.11\;\, 0.14\right]^T}$.}
\label{fig:traj}
\vspace{7.5pt}
\includegraphics[width=.99\linewidth]{images/navigation_biases_error}
\vspace{-20pt}
\caption{Log plot of the Equivariant error in \equref{local_coord_xi} for different initial conditions represented with different colors. $\epsilon_1$ represent the navigation error including position, attitude and velocity, while $\epsilon_2$ represent the biases error, including accelerometer, gyroscope and virtual velocity biases. Dots represent the initial values of the errors.}
\label{fig:logerrors}
\vspace{7.5pt}
\includegraphics[width=.99\linewidth]{images/lyapunov_small_2}
\vspace{-20pt}
\caption{Time evolution of the Lyapunov funtion (Filter energy) $\calL_t$ for different initialization of the filter, showing the exponential asymptotic convergence of the linearized error. The different colors represent the different initializations of the filter as shown in \figref{logerrors}.}
\label{fig:lyap}
\vspace{-17.5pt}
\end{figure}

\begin{figure}[!t]
\vspace{-5pt}
\centering
\includegraphics[width=0.99\linewidth]{images/trajectory_L1}
\caption{Real-world \ac{uav} Lissajous trajectory plot, showing in light green the ground-truth, in red and in blue the \ac{eqf} and \ac{ekf} estimate respectively. Note that, in this experiment, both filters were wrongly initialized with identity orientation, zero velocity and biases, and ${\prescript{G}{}{\hat{\bm{p}}}_{I} = \left[-1\;-1\;0.5\right]^T}$.}
\label{fig:real_world_trajectories}
%\vspace{-10pt}
\end{figure}

\begin{table}[!t]
\renewcommand{\arraystretch}{1.15}
\centering
\scriptsize
\caption{}
\vspace{-5pt}
\begin{tabular}{c c c c c}
\specialrule{.1em}{.1em}{.1em} 
\textsc{Rmse}  & Att [\si[per-mode = symbol]{\degree}]& Pos [\si[per-mode = symbol]{\meter}] & Vel [\si[per-mode = symbol]{\meter\per\second}] \\ \hline
\ac{eqf} & $\mathbf{1.978}$ & $\mathbf{0.0574}$ & $\mathbf{0.1180}$ \\
\ac{ekf} & $2.637$ & $0.0596$ & $0.1189$ \\
\specialrule{.1em}{.1em}{.1em} 
\end{tabular}
\label{tab:rmse_L}
\vspace{-10pt}
\end{table}

